Room Clearance with Feudal Hierarchical Reinforcement Learning

Reinforcement learning (RL) is a general framework that allows systems to learn autonomously through trial-and-error interaction with their environment. In recent years combining RL with expressive, high-capacity neural network models has led to impressive performance in a diverse range of domains. However, dealing with the large state and action spaces often required for problems in the real world still remains a significant challenge. In this paper we introduce a new simulation environment, "Gambit", designed as a tool to build scenarios that can drive RL research in a direction useful for military analysis. Using this environment we focus on an abstracted and simplified room clearance scenario, where a team of blue agents have to make their way through a building and ensure that all rooms are cleared of (and remain clear) of enemy red agents. We implement a multi-agent version of feudal hierarchical RL that introduces a command hierarchy where a commander at the higher level sends orders to multiple agents at the lower level who simply have to learn to follow these orders. We find that breaking the task down in this way allows us to solve a number of non-trivial floorplans that require the coordination of multiple agents much more efficiently than the standard baseline RL algorithms we compare with. We then go on to explore how qualitatively different behaviour can emerge depending on what we prioritise in the agent's reward function (e.g. clearing the building quickly vs. prioritising rescuing civilians).

==> sections/initial_draft_start.tex <==
\section{Introduction}
In multi-agent reinforcement learning, one of the main issues is the non-stationarity of the environment. To be more exact, for each individual agent, the environment looks highly non-stationary since the other agents are learning as well, so their behaviour cannot be caught by the learning agent. To account for this, communications between the agents is usually employed. In one of its flavours this is known as centralized training, decentralized execution. In this case there is a critic which integrates information from all agents, but only when training. When testing, or executing, this critic is not used anymore, but the agents learn to function in the same regime as in training even though there is no more integration of all agents' information.

We adopted another solution to this problem, which gives some other advantages as well, in the form of hierarchical reinforcement learning. One of the other reasons for adopting HRL is to use the tool we are developing for tactics or strategy finding and concept analysis in military applications. We would like to model a chain-of-command where higher-level commanders give orders to lower-level commanders which in turn give orders to agents which are acting in the environment, which we will call action agents. The commanders are purely virtual entities, and each one commands a subset of the ones below (valid for action agents as well). Other significant advantages of using HRL is the partitioning of the state-action space such that we don't have to deal with huge action spaces (assuming controlling all agents at once would mean a joint action space which grows exponentially in the number of agents) or act on large state spaces (assuming we integrate or concatenate all agents' states). By having small groups of agents controlled (here control means they receive a command which is then considered as part of the state) by one commander at the level above, and small groups of commanders controlled by one commander above, the overall efficiency of training would be significant. One more point for using HRL is the capability which such agents have when dealing with small differences in the environment, also known as transfer learning. How does learning transfer from one environment to the other, when the environment are somewhat similar. Partitioning the state-action space hierarchically allows to deal with such transfer learning in a more efficient manner.

\section{Environments}

We deal with 2 main types of environment. One is a capture-the-bomb environment, where the agents need to find an object of interest in a gridworld. This can be a very simple environment if the object stays fixed for all the training episodes, and if the number of rooms in the gridworld is small, or can be quite hard to achieve if the object of interest is moving in each episode and if the number of rooms is large. Basically is a shortest path problem, a toy problem, such that we can figure out how such agents compare with flat agents which have joint action spaces. The other environment is a room clearance environment, where agents need to clear a building comprising multiple rooms in such a way that enemies which might be hidden in some of the rooms will be uncovered. This requires that the agents discover a specific sequence of going into the rooms, as a function of the whole building topology (how rooms are connected through doors) such that the enemies cannot hide in any of the empty rooms.

\subsection{Room clearance}
This is an environment where we would like the agents to clear all the rooms in a building. Next, we define the concepts needed to understand the room clearance environment:
\begin{itemize}
\item{\textit{occupied room} is a room with one or more agents in it}
\item{\textit{unoccupied room} is a room with no agent in it}
\item{\textit{clear room} can be an occupied or unoccupied room, but which has no path to a unclear room if it's unoccupied}
\item{\textit{unclear room} is an unoccupied room which either has not been visited at all, or has been visited but has a path, without an occupied room on it, to an unclear room}
\end{itemize}
In short, every unclear room propagates the property to neighbouring rooms with no agents in them. This is modelled this way, assuming that in an unclear might be an enemy force which can then move to adjacent rooms, once no agent is in it. To find the unclear rooms we use the adjacency matrix of the room graph. The room graph represents the connections between rooms, if there's a door between one room and another, then we say they are connected. In computing which rooms are clear and which not we use the properties of the adjacency matrix with respect to multiplication. We know that by raising an adjacency matrix to the power $n$ we will then have on position $ij$ the number of paths of length n between nodes $i$ and $j$. Intuitively, the adjacency matrix propagates some (binary) property through multiplication, with one multiplication representing one additional step. We first denote the vector of \textit{unclear} rooms with $\textbf{u}$, the adjacency matrix with $\textbf{A}$ and the vector of unoccupied rooms with \textbf{v}. We can then get iterate through the next equation to get the unclear rooms:
\begin{equation}
  \textbf{u} = (\textbf{A} \times \textbf{u}) \cdot \textbf{v}
\end{equation}
Assuming the number of rooms is $m$, then vector \textbf{u} is size $m \times 1$, the matrix \textbf{A} is size $m \times m$ and the vector \textbf{v} is $m \times m$. The first multiplication with the matrix propagates one step the unclear rooms, and the multiplication with the unoccupied vector sets the rooms which have agents in them to clear, and is an element wise multiplication. As we are not interested in the number of paths, we clip the values obtained to 1s, to denote unclear. We reitarate this procedure (to simulate more steps) until the result is not changing from one step to the next, which means that the result, which is the unclear rooms vector is not changing with more steps. We will use the difference in the number of unclear rooms from one step to the next as reward shaping, if there are more clear rooms the reward will be positive, else the reward will be negative.
